Federated Learning with Heterogeneous Data Handling for Robust Vehicular Object Detection

In the pursuit of refining precise perception models for fully autonomous driving, continual online model training becomes essential. Federated Learning (FL) within vehicular networks offers an efficient mechanism for model training while preserving raw sensory data integrity. Yet, FL struggles with non-identically distributed data (e.g., quantity skew), leading to suboptimal convergence rates during model training. In previous work, we introduced FedLA, an innovative Label-Aware aggregation method addressing data heterogeneity in FL for generic scenarios. In this paper, we introduce FedProx+LA, a novel FL method building upon the state-of-the-art FedProx and FedLA to tackle data heterogeneity, which is specifically tailored for vehicular networks. We evaluate the efficacy of FedProx+LA in continuous online object detection model training. Through a comparative analysis against conventional and state-of-the-art methods, our findings reveal the superior convergence rate of FedProx+LA. Notably, if the label distribution is very heterogeneous, our FedProx+LA approach shows substantial improvements in detection performance compared to baseline methods, also outperforming our previous FedLA approach. Moreover, both FedLA and FedProx+LA increase convergence speed by 30% compared to baseline methods.

==> draft.tex <==
Related Work:

Zhao et al.~\cite{zhao2018federated} showed that the accuracy of \gls{FL} reduces significantly for neural networks trained for highly skewed \gls{non-IID} data, and proposed a strategy to improve training on \gls{non-IID} data by creating a small subset of data which is globally shared between all the edge devices.
Li et al.~\cite{li2019convergence} analyzed the effect of the \gls{non-IID} setting on the model performance when using \gls{FedAvg}, and showed how heterogeneity slows down the convergence.
FedAvgM~\cite{hsu2019measuring} proposed a method which aims to improve the model aggregation phase. Specifically, FedAvgM applies momentum when updating the global model on the server.
On the other hand, FedNova~\cite{wang2020tackling} normalizes the local updates before model aggregation.
More recently, FedProx~\cite{li2020federated} proposed to add a proximal term to the local subproblem to approximately limit the impact of variable local updates.
to help the model faster converge in statistically heterogeneous settings.
MOON~\cite{li2021model} introduced model-contrastive FL, correcting the local updates by maximizing the similarity of the representation learned by the local model and the representation learned by the global model.

To handle the heterogeneity when using \gls{FL} in the vehicular application,
Liu et al.~\cite{liu2022fed2a} proposed \gls{Fed2A} to reduce the direct effect of local parameters heterogeneity and improve the model performance by harnessing temporal and informative attributes of local parameters.
Their proposed aggregation scheme considers the \textit{freshness} of the received local models by using temporal weights, and \textit{consistency} by punishing stale models.
Shang et al.~\cite{shang2023fedbikd} proposed \gls{FedBiKD} framework to mitigate the issue of local deviation.
More specifically, in \gls{FedBiKD} the global knowledge is used to guide local training while using the common knowledge from the ensemble of local models to fine-tune the aggregated global model.
They evaluated their approach to the application of a training model for distracted driving detection and proved its superiority over FedProx and MOON.



--------------------------

To enable fully autonomous driving, the \gls{ADAS} must exhibit solid reliability across a spectrum of scenarios~\cite{van2018autonomous}.
%from sensors to environment models
Conventionally, sensory data collected from the vehicle's sensors, including \glspl{LiDAR}, Cameras, and Radars, is provided to perception models, such as \glspl{DNN}, to construct a thorough representation of the surroundings—a local environment model~\cite{liu2020computing}.
%issues of conventional training
The accuracy of this environmental model holds paramount significance in influencing the decision-making process for controlling the vehicle's behavior. 
However, relying solely on centrally training perception models with data obtained under constrained conditions falls short of ensuring reliability~\cite{schiegg2020collective}.
%continaus online training
To encounter these limitations and refine exceptionally precise perception models adaptable to diverse conditions, the imperative shift towards continuous online model training becomes apparent~\cite{khalil2022situational}.
This paradigm shift is crucial for the realization of a robust and dependable foundation towards fully autonomous driving.
\newline
%FL as a proper solution
\gls{FL} has recently emerged as a technique for enabling model training without necessitating the exchange of clients' data with a central entity during the training process~\cite{mcmahan2017communication, mammen2021federated, khalil2022situational}.
\begin{figure}[t]
\centering
    \includegraphics[width=0.3\textwidth]{Figures/1-intro/federated_dynamic_model_training.pdf}
\caption{Online training of the general perception model using \gls{FL} \cite{khalil2022situational}. At each communication round (1) Local updates are transmitted to the edge server (\eg \gls{RSU}), where intermediate aggregation takes place. (2) The edge servers transfer the aggregated model to the central aggregation server, which performs the final aggregation. (3) and (4) The aggregated model is then transferred back to the individual clients (vehicles).}
  \label{fig:FLForTraining}
  \vspace{-1.5em}
\end{figure}
\gls{FL} facilitates training on the available data distributed across clients at each communication round, as illustrated in Figure \ref{fig:FLForTraining}.
The local updates from clients are iteratively aggregated to converge towards the global optimum.
Significantly, these local updates are considerably smaller in size compared to the entirety of clients' data, a notable departure from the conventional model training paradigm where extensive data exchange is required.
\newline
The dual features of \gls{FL}, namely its ability to enable continuous online model training and its substantial reduction in exchanged data, position it as an ideal technique for training \gls{ML} models tailored for vehicular applications.
The use of \gls{FL} in vehicular networks has attracted significant attention in recent years~\cite{elbir2022federated, posner2021federated, chellapandi2023federated}.
Within vehicular networks, vehicles themselves serve as clients, generating data about their surrounding environment through their sensor sets.
This perception data is collaboratively utilized for training perception models, such as object detection models, without overwhelming the communication network with the burden of heavy sensory data.
Moreover, \glspl{RSU} or cloud servers can orchestrate the training process by initiating the trained model and aggregating the model updates received from vehicles during each communication round~\cite{pervej2023resource}.
\newline
%Heterogeneity issue
While \gls{FL} demonstrates effectiveness in scenarios with \gls{IID} data, it encounters challenges in achieving comparable performance when faced with data heterogeneity across clients, often referred to as \gls{non-IID} data~\cite{vahidian2023rethinking, ye2023heterogeneous}.
The various manifestations of \gls{non-IID} data were explored in our prior work~\cite{khalil2023label}, where we delved into distinct deviations from the \gls{IID} paradigm as outlined by Kairouz et al.~\cite{kairouz2021advances}.
In our comprehensive literature review, we addressed the adverse impact of \gls{non-IID} data on the training process. We categorized existing strategies into two main approaches: \textbf{Data-based approaches} and \textbf{Parameter-based approaches}.
One of our contributions, FedLA, was introduced as a data-based approach specifically designed to address the challenge of \textit{label distribution skew}. We conducted evaluations using common \gls{FL} datasets, providing empirical evidence of FedLA's performance in mitigating the impact of \gls{non-IID}ness.
\newline
%Contributions of Our Study
In this work, we extensively explore the existing literature concerning heterogeneity handling in vehicular network scenarios.
Moreover, we introduce FedProx+LA, a novel \gls{FL} method building upon FedProx to tackle the data heterogeneity issue.
FedProx+LA is a hybrid method that considers both data and the model's parameters
Additionally, we assess the effectiveness of FedLA and FedProx+LA in the context of online model training for object detection.
For the evaluation we conduct a comparative analysis against FedAvg~\cite{mcmahan2017communication} as a traditional aggregation method, the simplified FedAvgL, and FedProx~\cite{li2020federated} as a cutting-edge alternative.
Our analysis reveals the superior enhancement in the detection performance as well as the increased convergence rate exhibited by FedLA and FedProx+LA in comparison to FedAvg, FedAvgL, and FedProx, particularly in the context of a realistic vehicular perception dataset (Nuscenes).
This is highlighted by a substantial improvement in the detection performance measured by \gls{mAP} by 5\% and 6\% for FedLA and FedProx+LA accordingly.
The comprehensive source code, covering various data distribution scenarios and corresponding experimental results across different performance metrics, is openly accessible at: 
\footnote{\url{https://github.com}}
\newline
%The remainder
The subsequent sections of this paper are structured as follows: Section \ref{sec:hh} comprehensively reviews recent literature on addressing heterogeneity in the model training process within vehicular networks using \gls{FL}.
Additionally, we introduce FedProx+LA and a streamlined variant of FedLA, termed FedAvgL.
In Section \ref{sec:eval}, we conduct a comprehensive empirical assessment of FedLA and FedProx+LA, exploring their performance across diverse experimental configurations.
Finally, we conclude our work with Section \ref{sec:conc}.






